Construction Sequences and Certifying 3-Connectedness

Tutte proved that every 3-connected graph on more than 4 nodes has a contractible edge. Barnette and Gruenbaum proved the existence of a removable edge in the same setting. We show that the sequence of contractions and the sequence of removals from G to the K_4 can be computed in O(|V|^2) time by extending Barnette and Gruenbaum's theorem. As an application, we derive a certificate for the 3-connectedness of graphs that can be easily computed and verified.

==> Splittings.tex <==
A \emph{splitting} of a node is an inverse contraction with both endnodes of the new edge being of degree at least $3$. For constructions using Tuttes Wheel Theorem, i.\,e., constructions with edge additions and splittings, we get similar characterizations based on Seymours Splitter Theorem~\cite{Seymour1980}. These characterizations cover minors instead of subdivisions of $G$ and are therefore more general, since every subdivision in $G$ is a minor of $G$. On the other hand, the characterizations are weaker in the sense that they do not specify which minor in $G$ is chosen, whereas the subdivision in Theorem~\ref{constructions} is fixed in $G$. However, it is straightforward that Theorem~\ref{constructions} cannot be generalized to minors, e.\,g., on $3$-regular graphs having a minor with a node of degree $4$.

\begin{theorem}\label{constructionsseymour}
Let $G_i$ be a $3$-connected minor of $G$. Then (...dont forget Negami...)
\begin{align}
	&\ G \text{ is $3$-connected}\label{theoremitem1}\\
	\Leftrightarrow &\ \exists \text{ construction using splittings and~\ref{operation1}}\label{theoremitem4}\\
	\Leftrightarrow &\ \exists \text{ basic construction using splittings, \ref{operation1} and~\ref{operation2}}\label{theoremitem5}\\
%	\Leftrightarrow &\ \exists \text{ basic construction using splittings and~\ref{operation1}}\label{theoremitem4}\\
	\Rightarrow &\ \exists \text{ basic construction using splittings and \ref{operation1} or $G_i$ is a wheel that is}\notag\\
	&\ \text{ smaller than the biggest wheel minor in $G$~\cite{Seymour1980}}\label{theoremitem6}\\
	& \emph{(all constructions are non-additive, start with $G_i$ and end at $G$)}\notag
\end{align}
\end{theorem}
\begin{beweis}
The existence of each of the constructions~\eqref{theoremitem4} and~\eqref{theoremitem5} implies that $G$ has to be $3$-connected by Lemma~\ref{preserving} and the fact that splittings preserve $3$-connectedness. To the contrary, if $G$ is $3$-connected, Seymours Splitter Theorem yields~\eqref{theoremitem6}. We show that~\eqref{theoremitem1} and~\eqref{theoremitem6} implies \eqref{theoremitem4} and~\eqref{theoremitem5}. If the construction part of~\eqref{theoremitem6} exists, \eqref{theoremitem4} and~\eqref{theoremitem5} follow. Otherwise, $G_i$ is a wheel smaller than the biggest wheel minor in $G$ and we can enlarge this wheel step by step until it is the biggest wheel minor in $G$ and use the construction part of~\eqref{theoremitem6} from there. To enlarge it, we can either add iteratively a parallel spoke edge and get~\eqref{theoremitem4} by splitting the endnode on the rim or we allow the additional operation~\ref{operation2}, yielding~\eqref{theoremitem5}.
\end{beweis}

We note that Truemper~\cite[Thm. 7.3.5b]{Truemper1998} states a slightly more powerful variant of~\eqref{theoremitem4} (along with a polynomial time algorithm), in which the only non-basic operation is the edge addition performed immediately before applying a splitting on one of its endnodes without leaving parallel edges. This endnode can be assumed to have degree $3$ as otherwise the splitting can be applied without the edge addition.
